ESP: Extro-Spective Prediction for Long-term Behavior Reasoning in Emergency Scenarios

Emergent-scene safety is the key milestone for fully autonomous driving, and reliable on-time prediction is essential to maintain safety in emergency scenarios. However, these emergency scenarios are long-tailed and hard to collect, which restricts the system from getting reliable predictions. In this paper, we build a new dataset, which aims at the long-term prediction with the inconspicuous state variation in history for the emergency event, named the Extro-Spective Prediction (ESP) problem. Based on the proposed dataset, a flexible feature encoder for ESP is introduced to various prediction methods as a seamless plug-in, and its consistent performance improvement underscores its efficacy. Furthermore, a new metric named clamped temporal error (CTE) is proposed to give a more comprehensive evaluation of prediction performance, especially in time-sensitive emergency events of subseconds. Interestingly, as our ESP features can be described in human-readable language naturally, the application of integrating into ChatGPT also shows huge potential. The ESP-dataset and all benchmarks are released at https://dingrui-wang.github.io/ESP-Dataset/.

==> doc/table/ablation_vis.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{doc/figure/prediction_result.png}
\caption{Trajectory scenarios of ESP. For clear illustration, we only show 10-second-long sequences. Red trajectories belong to the target vehicles for which we will provide a prediction, and blue trajectories are generated by neighbors. Dotted lines denote lane centerlines. The ESP encoding mechanism proves to be highly valuable, yielding rapid and discernible improvements in model performance.}
\label{fig:ablation_vis}
\vspace{-0.3in}
\end{figure}

==> doc/table/cte_demo.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l l c c c c}
        \hline
        & Prediction example        & FDE           & ADE           & CTE        \\
        \hline
        & Prediction A              & \emph{2.33}   & \emph{1.00}   & \emph{1.30}   \\
        & Prediction B              & \emph{2.35}   & \emph{1.02}   & \emph{3.50}   \\
        \hline
    \end{tabular}
    \caption{Ablation Study concerning ESP Features for MTR Model with ESP Encoder equipped.}
    \label{tab:Ablation_Study_MTR}
\end{table}

\begin{figure}[htb]
\includegraphics[width=1.0\columnwidth]{doc/fig/CTE_metric_demo.pdf}
\caption{We employed the TNT-ESP model to evaluate a single token using different ESP inputs (as explained in the ablation study section). Among the findings, we obtained two prediction results that were similar in ADE and FDE but significantly different in the CTE metric.}
\label{fig:CTE_metric_demo}
\vspace{-2ex}
\end{figure}

==> fun.tex <==
\begin{table}[t] 
\caption{Comparison of popular behavior prediction and motion forecasting datasets. }
\label{tab:Comparison between datasets}
\centering
\begin{tabular}{cccccccccc} %需要10列
\toprule %添加表格头部粗线
\multicolumn{3}{c}{Dataset}&Boxes&Sampling rate&Time horizon&Interactions&Highway&Contextual info\\  %有n个&，就表示该行有n+1列
\hline %绘制一条水平横线
\multicolumn{3}{c}{Lyft Level 5\cite{kesten2019lyft}}&2D&10 Hz&5 s&{}&\checkmark & \\   % 占两列，列名为A；后面陆续跟着数字
\multicolumn{3}{c}{NuScenes\cite{caesar2020nuscenes}}&3D&2 Hz&6 s& & & \\
\multicolumn{3}{c}{Argoverse\cite{chang2019argoverse}}&None&10 Hz&3 s&{}&\checkmark & \\
\multicolumn{3}{c}{Interactions\cite{zhan2019interaction}}&2D&10 Hz&3 s&\checkmark & & \\
\multicolumn{3}{c}{WOMD\cite{ettinger2021large}}&3D&10 Hz&8 s&\checkmark & & \\
\multicolumn{3}{c}{Ours}&2D&10 Hz&\textbf{10 s}&\checkmark&\checkmark&\checkmark\\
\bottomrule %添加表格底部粗线
\end{tabular}
\end{table}


==> futher_author_info.tex <==
\author{Dingrui Wang$^*$$^{1}$, Zheyuan Lai$^{1}$, Yuda Li$^{1}$, Liang Ma$^{1}$, Ting Yu$^{1}$ and Wei Li\textsuperscript{†}$^{1}$
\thanks{$^{1}$Dingrui Wang, Zheyuan Lai, Yuda Li, Liang Ma, Ting Yu and Wei Li are with the Inceptio Technology Inc., China {\tt\small \{dingrui.wang, zheyuan.lai, yuda.li, liang.ma, ting.yu, wei.li\}@inceptio.ai}}%
\thanks{$^*$This work is done when Dingrui interned at Inceptio Technology Inc.}%
\thanks{\textsuperscript{†}This work is supported by the Inceptio Technology Inc. Corresponding author: Wei Li.}
}



Title options:
1. Beyond Trajectories: Unveiling Contextual Context-Aware for highway behavior prediction

2. "Context in Overdrive: Revving Up Autonomous Safety with the ESP-dataset

\begin{table*}[t] 
\caption{Comparison of popular behavior prediction and motion forecasting datasets. }
\label{tab:Comparison between datasets}
\centering
\begin{tabular}{ccccccccccccc} %需要10列
\toprule %添加表格头部粗线
\multicolumn{3}{c}{Dataset}&Average Vel (km/h)&$>$ 60 km/h&Boxes&Sampling rate&Time horizon&Interactions&Highway&Contextual info\\  %有n个&，就表示该行有n+1列shi
\hline %绘制一条水平横线
\multicolumn{3}{c}{Lyft Level 5\cite{kesten2019lyft}}&22.36&2.92\%&2D&10 Hz&5 s&{}&\checkmark \\   % 占两列，列名为A；后面陆续跟着数字
\multicolumn{3}{c}{NuScenes\cite{caesar2020nuscenes}}&23.24&0.09\%&3D&2 Hz&6 s\\
\multicolumn{3}{c}{Argoverse\cite{chang2019argoverse}}&34.72&6.51\%&None&10 Hz&3 s&{}&\checkmark\\
\multicolumn{3}{c}{Interactions\cite{zhan2019interaction}}&\textcolor{red}{(TBD)}&\textcolor{red}{(TBD)}\%&2D&10 Hz&3 s&\checkmark\\
\multicolumn{3}{c}{WOMD\cite{ettinger2021large}}&\textcolor{red}{(TBD)}&\textcolor{red}{(TBD)}\%&3D&10 Hz&8 s&\checkmark&\\
\multicolumn{3}{c}{Ours}&\textbf{56.68}&\textbf{40.43}\%&2D&10 Hz&\textbf{10 s}&\checkmark&\checkmark&\checkmark\\
\bottomrule %添加表格底部粗线
\end{tabular}
\end{table*}

Rewrite text below to make it both easy to understand for a non-native English speaker and similar to text on a paper on International Conference on Robotics and Automation:" 
We review a range of datasets and highlight the unique- ness and the relationship between the current datasets and the proposed dataset.
 
 " 

\begin{table}[h]
    \centering
    \begin{tabular}{l c c c c}
        \hline
        & Model &Precision & Recall & Accuracy \\

        \hline
        & LSTM (with traj.) & \emph{0.70} & \emph{0.73} & \emph{0.65} \\
        
        & LSTM (with esp.) &  \emph{0.80} & \emph{0.85} & \emph{0.78} \\

        & LSTM (with esp. \& traj.) & \emph{0.83} & \emph{0.89} & \emph{0.82} \\
         %& GPT-4 (Langchain-based) & \emph{-} & \emph{-} & \emph{-} & \emph{0.30} & \emph{1.00} & \emph{0.30} \\
        \hline
    \end{tabular}
    \caption{Benchmark Results for Front Blocking Scenario}
    \label{tab:front_blocking_results}
\end{table}


\begin{table*}[t]
    \centering
    \begin{tabular}{l l c c c c c c}
        \hline
        & Model                                           & minFDE        & minADE        & minCTE        & Precision     & Recall        & Accuracy \\
        \hline
        & MTR-ESP (with all ESP features)             & \emph{4.33}   & \emph{2.00}   & \emph{0.71}   & \emph{0.75}   & \emph{0.83}   & \emph{0.76} \\
        & MTR-ESP-retrained (w/o tv-ev)               & \emph{4.89}   & \emph{2.21}   & \emph{0.74}   & \emph{0.73}   & \emph{0.83}   & \emph{0.75} \\
        & MTR-ESP-retrained (w/o tv-cipv)             & \emph{5.22}   & \emph{2.32}   & \emph{0.75}   & \emph{0.75}   & \emph{0.80}   & \emph{0.75} \\
        & MTR-ESP-retrained (w/o ego-tv)              & \emph{5.88}   & \emph{2.59}   & \emph{0.82}   & \emph{0.72}   & \emph{0.78}   & \emph{0.72} \\
        & MTR-ESP-retrained (w/o ego-cipv)            & \emph{4.87}   & \emph{2.20}   & \emph{0.74}   & \emph{0.73}   & \emph{0.83}   & \emph{0.74} \\
        & MTR-ESP-retrained (w/o ego-ev)              & \emph{5.23}   & \emph{2.33}   & \emph{0.75}   & \emph{0.72}   & \emph{0.82}   & \emph{0.74} \\
        & MTR-ESP-retrained (w/o all ESP features)    & \emph{5.21}   & \emph{2.33}   & \emph{0.75}   & \emph{0.74}   & \emph{0.81}   & \emph{0.34} \\
        \hline
    \end{tabular}
    \caption{Ablation Study concerning ESP Features for MTR Model with ESP Encoder equipped.}
    \label{tab:Ablation_Study_MTR}
\end{table*}

\begin{table*}[t] 
\label{tab:Comparison_between_datasets}
\centering
\begin{tabular}{lccccccccc} %需要10列
\toprule
\multicolumn{3}{c}{}                        &NuSc       &Argo             &Inter          &WOMD            &HDD            &Ours           \\ 
\hline
\multicolumn{3}{c}{Boxes}                   &3D         &None             &2D             &3D              &2D             &2D            \\  
\multicolumn{3}{c}{Time horizon}            &6 s        &3 s              &3 s            &8 s             &5 s            &5 s           \\
\multicolumn{3}{c}{Segments}                &1k         &324k             &{-}            &104k            &120k           &120k          \\
\multicolumn{3}{c}{Segment duration}        &20 s       &5 s              &{-}            &20 s            &10 s           &10 s          \\
\multicolumn{3}{c}{Density of aggressive 
behavior}                                   &low        &low              &high           &low             &low            &very high          \\
\multicolumn{3}{c}{Unique road ways}        &{-}        &290 km           &{-}            &1750 km         &2000 km        &2000 km       \\
\hline
\multicolumn{3}{c}{Sampling rate}           &2 Hz       &10 Hz            &10 Hz          &10 Hz           &10 Hz          &10 Hz          \\
\multicolumn{3}{c}{obejct types}            &1          &1                &1              &3               &4              &4             \\
\multicolumn{3}{c}{HD map}                  &{}         &\checkmark       &{}             &\checkmark      &\checkmark     &\checkmark    \\
\multicolumn{3}{c}{Interactive features}    &{}         &{}               &\checkmark     &\checkmark      &\checkmark     &\checkmark    \\
\multicolumn{3}{c}{highway}                 &{}         &{}               &\checkmark     &\checkmark      &\checkmark     &\checkmark    \\
\multicolumn{3}{c}{Close Junction}          &{}         &{}               &{}             &{}              &{}             &\checkmark    \\
\multicolumn{3}{c}{Speed Monitor}           &{}         &{}               &{}             &{}              &{}             &\checkmark    \\
\multicolumn{3}{c}{Rare road objects}       &{}         &{}               &{}             &{}              &{}             &\checkmark    \\
\bottomrule 
\end{tabular}
\caption{Comparison of popular behavior prediction and motion forecasting datasets including
NuSc\cite{caesar2020nuscenes}, Argo\cite{chang2019argoverse}, Inter\cite{zhan2019interaction}, WOMD\cite{ettinger2021large}.}
\end{table*}
